Cost-Recovering Bayesian Algorithmic Mechanism Design

We study the design of Bayesian incentive compatible mechanisms in single parameter domains, for the objective of optimizing social efficiency as measured by social cost. In the problems we consider, a group of participants compete to receive service from a mechanism that can provide such services at a cost. The mechanism wishes to choose which agents to serve in order to maximize social efficiency, but is not willing to suffer an expected loss: the agents' payments should cover the cost of service in expectation. We develop a general method for converting arbitrary approximation algorithms for the underlying optimization problem into Bayesian incentive compatible mechanisms that are cost-recovering in expectation. In particular, we give polynomial time black-box reductions from the mechanism design problem to the problem of designing a social cost minimization algorithm without incentive constraints. Our reduction increases the expected social cost of the given algorithm by a factor of O(log(min{n, h})), where n is the number of agents and h is the ratio between the highest and lowest nonzero valuations in the support. We also provide a lower bound illustrating that this inflation of the social cost is essential: no BIC cost-recovering mechanism can achieve an approximation factor better than \Omega(log(n)) or \Omega(log(h)) in general. Our techniques extend to show that a certain class of truthful algorithms can be made cost-recovering in the non-Bayesian setting, in such a way that the approximation factor degrades by at most O(log(min{n, h})). This is an improvement over previously-known constructions with inflation factor O(log n).

==> app-bic.tex <==
\section{Omitted proofs from Section~\ref{SEC:BIC}}
\label{app:app-bic}
%\begin{oneshot}{Claim~\ref{cl:log-n}}
%Given $k$ real numbers $a_1,\dots, a_k$, such that $a_i \geq 1$ for all $i$, 
%$\sum_{j=1}^{k} \frac{a_j}{\sum_{t\geq j} a_t} \leq 2\cdot H_{\sum_{j=1}^{k}\lfloor a_j \rfloor },$
%where $H_r = \sum_{i=1}^{r} \frac{1}{i} = 1+ \log r$. 
%\end{oneshot} 
\begin{proof}
\begin{align*}
\sum_{j=1}^{k} \frac{a_j}{\sum_{t\geq j} a_t} &= \sum_{j=1}^{k} \frac{\lfloor a_j\rfloor}{\sum_{t\geq j} a_t} + 
\sum_{j=1}^{k} \frac{a_j - \lfloor a_j\rfloor}{\sum_{t\geq j} a_t}\\
&\leq \sum_{j=1}^{k} \frac{\lfloor a_j\rfloor}{\sum_{t\geq j} \lfloor a_t \rfloor } + \sum_{j=1}^{k} \frac{1}{\sum_{t\geq j} a_t}\\
&\leq \sum_{j=1}^{k} \frac{\lfloor a_j\rfloor}{\sum_{t\geq j} \lfloor a_t \rfloor } + H_k \\
&\leq \sum_{j=1}^{k} \frac{\lfloor a_j\rfloor}{\sum_{t\geq j} \lfloor a_t \rfloor } + H_{\sum_{j=1}^{k}\lfloor a_j\rfloor}
\end{align*}

We now show that $\sum_{j=1}^{k} \frac{\lfloor a_j\rfloor}{\sum_{t\geq j} \lfloor a_t \rfloor } \leq H_{\sum_{j=1}^{k}\lfloor a_j\rfloor}.$
We drop the floors, and assume that the $a_j$'s are integers in the part below. Consider the term $\frac{a_j}{\sum_{t\geq j} a_t}.$
\begin{align*}
\frac{a_j}{\sum_{t\geq j} a_t} &= \underbrace{\frac{1}{a_j+a_{j+1}+\ldots+a_{k}}+\ldots+\frac{1}{a_j+a_{j+1}+\ldots+a_{k}}}_{a_j \text{ times}}\\
&\leq \frac{1}{1+a_{j+1}+\ldots+a_{k}}+\frac{1}{2+a_{j+1}+\ldots+a_{k}}+\ldots+\frac{1}{a_j+a_{j+1}+\ldots+a_{k}}\\
&= \sum_{t=1+\sum_{k> j}a_k }^{a_j+\sum_{k> j}a_k}\frac{1}{t}
\end{align*}

So we have,
\begin{align*}
\sum_{j=1}^{k} \frac{a_j}{\sum_{t\geq j} a_t} \leq \sum_{j=1}^{k} \sum_{t=1+\sum_{k> j}a_k}^{\sum_{k\geq j}a_k}\frac{1}{t} = \sum_{t=1}^{\sum_j a_j}\frac{1}{t} = H_{\sum_j a_j}
\end{align*}
\end{proof}



==> b01.tex <==
Given an algorithm $A$ that gives a $\rho$-approximation to the purely
algorithmic social-cost minimization problem, we give a simple reduction that uses $A$
as a black-box and produces a truthful cost-recovering mechanism $CM$ that gives a
$\rho$-approximation to the social cost minimization problem. 
%Thus for $0/1$ valuation problems, this is an improvement from the $O(\rho\log n)$
%approximation of Georgiou and Swamy~\cite{GS12}. 
Further we do not place any
restrictions on what kind of algorithm $A$ should be. 

\begin{enumerate}
\item Let $S(\vals)$ be the set returned by $A$ on input $\vals$. 
\item Let $S'(\vals) \leftarrow S(\vals)\setminus D(\vals)$, where $D(\vals) = \{i\in S| v_i = 0\}$
\item If $C(S'(\vals)) \leq |S'(\vals)|$ return $S'(\vals)$ as the outcome, with a price of $1$ for
each agent
\item Else return $\emptyset$ as the outcome
\end{enumerate}

The above mechanism can be clearly seen to be truthful: a zero agent never wins,
so a 1-agent will not pretend to be zero. A 1-agent always gets a zero utility,
so a zero-agent is indifferent between reporting zero and 1. The operations
involved only reduce cost: $|S'(\vals)| \leq |S(\vals)|$, and the case where we return
$\emptyset$ is also cost reducing. 


==> ep_k.tex <==
\subsection{Black-box reduction for valuations of support $k$}
\label{sec:ep-k}

Suppose the support of the
agents' valuations are known, and have a support size of $k$, given by $\left\{\vali[1],\dots,\vali[k]\right\}$. 
From the proof of Theorem~\ref{thm:ep_general} it follows that we can obtain a $O(\rho\log k)$ approximation by
proceeding the cost recovery through each value in the support in the ascending order, rather than in powers of two. The factor of $\log h$, gets improved to a factor of $k$. We have the following corollary. 
\begin{corollary}
Given a truthful no-bossy mechanism that minimizes social cost to a factor of 
$\rho$, and when the valuations of all agents reside in $\left\{\vali[1],\dots,\vali[k]\right\}$,
there exists an efficiently computable black-box reduction that outputs a mechanism that minimizes social
cost to a factor of $O(\rho k)$, and recovers cost. 
\end{corollary}


